Video Harness: Evidence-Constrained Video Editing with Agentic Search

An informative video needs both a well-informed narrative and footage that can carry it. We propose Video Harness, an agent framework that combines adaptive agentic search with narration-first planning. Its central idea is to establish what the video should communicate before selecting what it should show. Multi-step search supplies source-grounded knowledge when research offers a clear benefit, and the complete narration script N is written before footage acquisition. The script becomes a blueprint for global shot assignment, where visual support, measured narration timing, and footage-reuse constraints jointly determine the edit. Capacity and conflict diagnostics guide targeted footage retrieval and targeted script revision to satisfy narrative and timing requirements. Evaluated against four systems on shared prompts, Video Harness achieves the highest overall automated score. Across prompts spanning five content-oriented prompt types, Video Harness outperforms Crayotter, the strongest baseline, by 18.24 points in mean prompt fulfillment. In the paired search-on/off comparisons, enabling search improves the mean score by 7.62 points, with a 29.05-point gain on news prompts.

==> cuhk-title.tex <==
% Public arXiv title page for the CVPR 2027 author kit.
\makeatletter
\newcommand{\maketitlewithteaser}[1]{%
  \iftoggle{cvprfinal}
    {\def\vh@teaserfile{#1}\maketitle}
    {\maketitle\input{#1}}%
}
\newcommand{\vh@inlinefigure}[1][]{\ignorespaces}
\iftoggle{cvprfinal}{%
  \renewcommand{\@maketitle}{%
    \vspace*{-18pt}
    \noindent\includegraphics[width=.25\textwidth]{fig/cuhk-logo2.png}\par
    \vskip 4pt
    \hrule height .7pt
    \vskip 5pt
    {\centering
      {\Large\bfseries \@title\par}%
      \vskip 8pt
      {\large\begin{tabular}{@{}c@{}}\@author\end{tabular}\par}%
    }%
    \ifdef{\vh@teaserfile}{%
      \vskip 14pt
      \nointerlineskip
      \hbox{\begin{minipage}{\textwidth}
        \centering
        \captionsetup{type=figure}%
        % The title is already full-width. Keep the original artwork,
        % caption and label, and typeset its outer wrapper in place.
        \let\strip\vh@inlinefigure       \let\endstrip\relax
        \let\figure\vh@inlinefigure      \let\endfigure\relax
        \cslet{figure*}\vh@inlinefigure  \cslet{endfigure*}\relax
        \renewenvironment{center}{\par\centering}{\par}%
        \input{\vh@teaserfile}%
      \end{minipage}}%
    }{}%
  }%
}{}
\makeatother

